Slow-growth approximation for near-wall patch representation of wall-bounded turbulence

Wall-bounded turbulent shear flows are known to exhibit universal small-scale dynamics that are modulated by large-scale flow structures. Strong pressure gradients complicate this characterization, however; they can cause significant variation of the mean flow in the streamwise direction. For such situations, we perform asymptotic analysis of the Navier-Stokes equations to inform a model for the effect of mean flow growth on near-wall turbulence in a small domain localized to the boundary. The asymptotics are valid whenever the viscous length scale is small relative to the length scale over which the mean flow varies. To ensure the correct momentum environment, a dynamic procedure is introduced that accounts for the additional sources of mean momentum flux through the upper domain boundary arising from the asymptotic terms. Comparisons of the model's low-order, single-point statistics with those from direct numerical simulation and well-resolved large eddy simulation of adverse-pressure gradient turbulent boundary layers indicate the asymptotic model successfully accounts for the effect of boundary layer growth on the small-scale near-wall turbulence.

==> small_scale_energy_results.tex <==
Filter 2d Euu and show universality in small scales

Show accumulation in $(k_x,k_z) = (0,1)$ for increasing
$dP^+/dx^+$. Because youre packing more and more 
energy into the same size box. 

Show or mention $\beta=3$ case to show it's not just unique  
to $\epsilon\ne0$. Actually, $\epsilon$ terms reduce wall
shear stress variance. 


==> time_integration_of_f.tex <==
The evolution of the streamwise $(k_x,k_z) = (0,0)$ Fourier mode $\overline{u}$ in the slow-growth model is 
\begin{equation}\label{eq:eq_motion_ubar2}
\pderiv{\overline{u}}{t} + \pderiv{}{y}\overline{uv} 
+ \epsilon_L \Big(\overline{uu} + \pderiv{}{y} (y\, \overline{uu})\Big) - \nu \frac{\partial^2 \overline{u}}{\partial y^2} 
=  f-\frac{dP}{dx},
\end{equation}
where $f(y,t) = \psi(t) g(y)$, and $g$ and $\psi$ are defined by \eqref{eq:g_defn} 
and \eqref{eq:psi_constraint}, respectively. Since $\psi$ depends on $\overline{uu}$, 
it treated explicitly in the third-order Runge-Kutta
time marching scheme \citep{Spalart:1991wu}. 

Let $\alpha_i$, $\beta_i$, $\gamma_i$, and $\zeta_i$ denote the RK coefficients at each RK substage, $i=1$, $2$, or $3$, and 
let the superscript $i$ denote the value of a time-dependent quantity at that substage. 
 Using semi-discrete notation (where derivative operators are written in continuous form), 
\eqref{eq:eq_motion_ubar2} is then discretized in time as
\begin{align}\label{eq:discrete_cbar}
\left(1 - \Delta t \beta^i \frac{\partial^2}{\partial y^2}\right) \overline{u}^{i+1} = \overline{u}^{i} 
&+ \Delta t \alpha^i \frac{\partial^2}{\partial y^2} \overline{u}^i \nonumber\\
&- \gamma^i \Delta t  \left( \pderiv{}{y} \overline{uv}^{i} 
+ \epsilon \, \overline{uu}^i + \epsilon \pderiv{}{y} (y\, \overline{uu}^{i})  - \psi^i g\right) \nonumber\\
&-\zeta^i \Delta t \left( \pderiv{}{y} \overline{uv}^{i-1} 
+ \epsilon \, \overline{uu}^{i-1} + \epsilon \pderiv{}{y} (y\, \overline{uu}^{i-1})  
- \psi^{i-1} g\right) \nonumber \\
&- (\gamma^i + \zeta^i)\Delta t \,\frac{dP}{dx} , 
%+ \epsilon \left( \pderiv{\left(y \overline{uu} \right)}{y} + \overline{uu} \right) = f(y,t) - \frac{dP}{dx}. 
\end{align}
where it is noted that $\zeta_1=0$. 
%The fully discrete equation written in B-spline space is: 
%\begin{align}
%\underbrace{\left(B_0 - \Delta t \beta^i B_2\right)}_{:= M} c_{\overline{u}}^{i+1} = \overline{u}^{i} &+ \Delta t \alpha^i \frac{\partial^2}{\partial y^2} \overline{u}^i 
%- \gamma^i \Delta t  \left( \pderiv{}{y} \overline{uv}^{i} 
%+ \epsilon \pderiv{}{y} (y \overline{uu}^{i}) + \epsilon \, \overline{uu}^i -\psi\big(\overline{uu}^i\big) \widetilde{f}\right)  \\
%&-\zeta^i \Delta t \left( \pderiv{}{y} \overline{uv}^{i-1} 
%+ \epsilon \pderiv{}{y} (y \overline{uu}^{i-1}) + \epsilon \, \overline{uu}^{i-1}-\psi\big(\overline{uu}^{i-1}\big) \widetilde{f} \right) \nonumber \\
%&- (\gamma^i + \zeta^i)\Delta t \, \frac{dP}{dx}, \nonumber 
%\end{align}
%where 
%\begin{equation}
%\psi\big(\overline{uu}^i\big) = \tau_{\rm tot} + \epsilon \left( L_y \overline{uu}^i_{N_y} + \vartheta \cdot B_0^{-1} \overline{uu}^i\right)
%\end{equation}
%when discretized. The $N_y$ subscript denotes the final element of the array, corresponding to the location $y=L_y$. 

